Augmented Bayesian Policy Search

Deterministic policies are often preferred over stochastic ones when implemented on physical systems. They can prevent erratic and harmful behaviors while being easier to implement and interpret. However, in practice, exploration is largely performed by stochastic policies. First-order Bayesian Optimization (BO) methods offer a principled way of performing exploration using deterministic policies. This is done through a learned probabilistic model of the objective function and its gradient. Nonetheless, such approaches treat policy search as a black-box problem, and thus, neglect the reinforcement learning nature of the problem. In this work, we leverage the performance difference lemma to introduce a novel mean function for the probabilistic model. This results in augmenting BO methods with the action-value function. Hence, we call our method Augmented Bayesian Search~(ABS). Interestingly, this new mean function enhances the posterior gradient with the deterministic policy gradient, effectively bridging the gap between BO and policy gradient methods. The resulting algorithm combines the convenience of the direct policy search with the scalability of reinforcement learning. We validate ABS on high-dimensional locomotion problems and demonstrate competitive performance compared to existing direct policy search schemes.

==> rebuttals/R1.tex <==
> (1) It is never explained the type of policy being used. / The derivation is based on nonparametric (tabular) policies, but those type of policies are too limited for the MuJoCo experiments. / Even the linear policy seems to be very limited.


We apologize for the possible lack of clarity in the paper that might have led to this confusion. We have updated the paper to clarify that our theoretical results apply to all kinds of policies.

RL with deterministic linear policies is a standard benchmark for the Bayesian optimization setting [1,2,3]. Indeed, for computational considerations, BO cannot easily scale to the thousands of dimensions required for a neural network actor. At least, not with the standard algorithms.

In our case, like in previous works, e.g., MPD and ARS, we show that linear policies are not too limiting for the MuJoCo experiments, as clearly evidenced by our successful experimental results. 

Our long-term goal is for Bayesian optimization to also scale to the larger neural network parameterizations of the policy, and we think that our proposed mean function that bridges a gap between BO and policy gradient methods is a good first step towards this goal.

> (2) The idea of incorporating information from x at theta is interesting, but that still requires to sample rollouts from the policy pi_x, which seems counterintutive in a BO setting where sample efficiency is of paramount importance.

We want to point out that this is a misunderstanding. Indeed, the returns and occupation measures of the policies $\pi_x$ used for the validation come from the already collected data. We make this point clearer in our update of Section 4. Thank you for your feedback.

> (3) It seems that the philosophy behind the mean function is similar to having a GP with inducing points. The other advantage of using pi_x seems exploration, but that can also be achieved with importance sampling.
Given the nature of the application (sample efficient PS), the authors should include in the comparison both novel AC methods (SAC, TQC…), model based approaches which are also sample efficient (MBPO…). For example, according to the MBPO paper [A], MBPO is able to achieve 6000 reward in a similar number of steps than ABS gets 4000.


 We kindly point out that the aim of our paper is to construct an effective algorithm for RL that explores using only deterministic policies. As cited in our introduction, we consider the problem of continuous MDPs. As for SAC, MBPO, and other bootstrapping-based methods, they do not fit into our problem of performing exploration using only deterministic policies, as mentioned in our abstract.


> (4) In the paragraph before eq 8, it says “Proposition 3.3”. I think you mean “Theorem 3.3”

Thank you for pointing this out. We fixed the reference.

> (5) Why all the policies in Figs 3 and 4 are normalized?

> (6) What do you mean by discounted policy returns? It seems that the undiscounted returns like the ones presented in the appendix are more standard in the literature and allows comparisons with other works.

In Figure 3,  we choose to report the discounted policy returns. Indeed, the RL agent is trying to optimize the discounted returns. Hence, we believed it would make more sense to report these. Since we report discounted returns, we believed that reporting the normalized values would allow for easier comparison. Finally, having noticed that certain policies have high discounted returns and a relatively lower undiscounted return (e.g. Hopper), we opted to report the undiscounted returns in the appendix in Figure (5) for more transparency and ease of comparison with other works. 


> (7) Also, the standard approach is to use steps for the horizontal axis, instead of episodes.

We report the policy return as a function of the number of episodes because direct policy search methods require rollouts of entire episodes. The majority of the literature of BO applied in RL uses this metric as a measure of their empirical sample efficiency [1,2,3]. In our experiments, all the tasks have a fixed horizon of 1000 steps.

> (8) The R2 analysis is unclear. The fact that for many iterations the correlation is negative and it is mostly below 0.5 means that the fitness might not be accurate. Furthermore, the R2 is a fitness measurement for linear regression, which does not seem to be the case for the Q-function.

We kindly point out that the R2 factor is a general metric to quantify the goodness-of-fit in regression, and is not only restricted to linear regression. 

We do not claim that the Q-function is always accurate. On the contrary, our results show large fluctuations in the validation metric at times. 

However, the validation metric has a median of over $50 \%$ for all the tasks. This means that the Q-function approximators are effective in reconstructing the returns of the last 3 batches of acquisition points that we choose to validate on. 

As for the test R2 score, it is as well consistently positive with medians of $> 50 \%$ for the "Ant" and "Halfcheetah" tasks. 

For "Walker2d", it seems to be harder to get a good test metric as the test R2 score has a median of $-20\%$. This is probably due to the lack of smoothness of the "Walker2d" making the residual terms higher, and thus, harder for our mean function to fit even with a perfect Q-function estimator. However, despite this, we see a large increase in the performance in "Walker2d" compared to the MPD baseline proving that we do not need the mean function to be a perfect predictor of the whole neighborhood but we need it just to identify a few good search directions.

To make the comprehension of results in Figure (2) easier, we make the following modifications: 

(a) We remove the averaging that was used to make the plots more readable and report the histograms of the distributions of the scores in the Appendix.
(b) We report the distributions and median of the scores in Figure (6) in the appendix.

> (9) Policy search with Bayesian optimization has been extensively studied since 2007 [B] and there are many works missing. For example, [C] presented a PS method with BO using local models as well, while [D] also combines parametric and non-parametric (GP) models.

Thanks for the references. We have added the citations.

[1] Müller, Sarah, Alexander von Rohr, and Sebastian Trimpe. "Local policy search with Bayesian optimization." Advances in Neural Information Processing Systems 34 (2021): 20708-20720.

[2] Nguyen, Quan, et al. "Local Bayesian optimization via maximizing probability of descent." Advances in neural information processing systems 35 (2022): 13190-13202.

[3] Eriksson, David, et al. "Scalable global optimization via local Bayesian optimization." Advances in neural information processing systems 32 (2019).


==> rebuttals/R2.tex <==
### Reviewer 2 ###

> (1) There is no comparison with one of the frequently used model-free RL methods with bootstrapping. Why was a comparison with bootstrapping-based methods such as NFQ [4], DQN [5], SAC [6], etc. omitted?

We kindly point out that the aim of our paper is to construct an effective algorithm for RL that explores using only deterministic policies. It is an important property of policy search methods, such as Bayesian optimization or random search, when applied to physical systems as discussed in the introduction of our paper. As also cited in our introduction, we consider the problem of continuous MDPs. Hence, methods like NFQ and DQN do not apply.

As for SAC and other bootstrapping-based methods, they do not fit into our problem of performing exploration using only deterministic policies, as mentioned.

> (2) The presentation does not classify the approach clearly enough in the very broad field of RL algorithms.

We improved the introduction section to better stress the use case of our algorithm. In broad terms, in this paper, we are interested in policy search algorithms that only execute deterministic policies on the controlled system. This includes two main classes: random search algorithms and Bayesian optimization. MPD, which our work builds on, is a Bayesian optimization algorithm and our main competitor in the experiments. One important contribution of our paper is that neural Q-functions can be used to improve the probabilistic modeling of Bayesian optimization. To support this statement, we have shown that our algorithm outperforms MPD on all the tasks.

> (3) The results do not show a clear superiority over the two comparative methods.

We would like to point out that our algorithm consistently outperforms the MPD baseline, which, to the best of our knowledge, is the state-of-the-art algorithm in BO for RL. Because our improvements are only on the probabilistic modeling of the policy return but not other components of BO, such as the acquisition function, we think that our proposed mean function can potentially improve many future BO methods when applied for RL, which we consider as our main contribution.

Also, we want to point out, that albeit performing slightly worse than ARS in Hopper and Halfcheetah, but we outperform all the competing algorithms by a large margin for Walker2d and Ant.

> (4) The method is only tested on deterministic MDPs without mentioning this limitation.

We raise the point that the majority of BO works applied in RL for continuous MDPs use the MuJoCO benchmark. Nevertheless, we want to remark that our theoretical results apply for both deterministic and stochastic MDPs. 

The fundamental challenges of learning in stochastic and deterministic MDPs with deterministic policies are similar in nature. For stochastic MDPs, due to much noisier evaluations, one can use more samples to construct the empirical estimates (e.g., policy return and discounted state occupation measure).

> (5) The term "deterministic exploration" requires an explanation.

Indeed, we fixed this in the introduction. Thank you for pointing this out.

> (6) Regarding "deterministic policy gradient, which changes its actions to maximize Qπθ (Silver et al., 2014)", I would like to note that this principle was already introduced in 2007 in [1].

We want to kindly point out that the aforementioned paper did not formally justify the use of the policy gradient for deterministic policies. This was initially introduced in the "Deterministic policy gradient" paper (Silver et al., 2014).

> (7) "max" should not be italicized, see Algorithm 1.

We fixed that. Thank you for your comment.

> (8) The sentence "Evolution of the validation and test scores a representative seed on the MuJoCo task" is incomprehensible.

It should have read "Evolution of the validation and test scores of a representative seed on the MuJoCo task". We have fixed that. Thank you for your feedback.

> (9) The claim "Our learned Q-function can reconstruct the real Q-function" is, in my opinion, not sufficiently substantiated by Figure 2.

We agree with the reviewer that this statement is inaccurate. We decided to remove this claim from the revised version.

> (10) In my opinion, "In the direct policy search literature, an alternative to BO is the use of Evolutionary Strategies" lacks the mention of the use of swarm-based methods such as PSO in [2] and [3].

Thank you. We have added these citations in the related works section of the revised paper.

> (11) There are several unintentional lower case letters in the references: bayesian, gaussian, lipschitz, markov.

Thank you for pointing this out. We have fixed this.

> (12) Why was a comparison with a bootstrapping-free, model-based method such as PILCO  omitted?

To the best of our knowledge, there has been no prior work that successfully applied PILCO on MuJoCO locomotion tasks, and prior work also noted more generally the lack of success of model-based methods using Gaussian processes for locomotion with frictional contacts [1] such as the MuJoCO tasks we consider.

[1]: Nagabandi, Anusha, et al. "Neural network dynamics for model-based deep reinforcement learning with model-free fine-tuning." 2018 IEEE international conference on robotics and automation (ICRA). IEEE, 2018.

[2]: Deisenroth, Marc Peter, et al. "Toward fast policy search for learning legged locomotion." 2012 IEEE/RSJ International Conference on Intelligent Robots and Systems. IEEE, 2012.


==> rebuttals/R3.tex <==
### Reviewer 3 ###

> (1) Minor: The plots can be improved, figure 2-4 is not very pretty (too high linewidth, scrollbar on the right, grid overrides plot)

Thank you for pointing this out. We have updated the figures now. Let us know if the updated figures are well suited. 

> (2) Performance is only marginally better/worse than existing methods

We point out that our algorithm consistently outperforms the MPD baseline, which, to the best of our knowledge, is the state-of-the-art algorithm in BO for RL. By doing so, we argue that our mean function can improve all potential future BO methods when applied for RL which would be more the takeaway message. Also, we would like to point out that despite performing slightly worse than ARS in Hopper and Halfcheetah, the gap between our method and ARS is never large in ARS' favor. In contrast, on the higher dimensional tasks that are Walker2d and Ant, our method largely outperforms ARS.

> (3) I believe a stronger case can be made if you would look at the method from a risk-sensitive perspective.

Thank you for raising this interesting point. We believe this is a promising direction that we aim to explore in future works. We refer the Reviewer to our response to point 5.B for additional discussion on the risk-sensitive perspective.

> (4) Your covariance function will only be a function of the standard kernel function. 

Thank you for raising another interesting point. As we mention in our conclusion, the kernel function is a direction we plan to explore for future works.

> (5) Did you see that compared to the baseline your approach gave a more stable/monotonic improvement over time?

When observing individual seeds, we did not notice more monotonic behavior of our algorithm compared to MPD and ARS for both the acquisition phase and when comparing the return from one central point to the other. Our explanation for this is threefold: 

A) The gradient of ARS can be seen as that of a robust optimization objective which justifies a fairly good monotonic increase. The same applies to MPD, which follows the maximum descent direction and hence demonstrates quite a consistent increase.

B) Another phenomenon is that the acquisition function is symmetric w.r.t to the posterior of the gradient $\mu_\theta$. Knowing that the direction $-d$ is bad is equivalent to knowing that direction $+d$ is good. Breaking the symmetry of the acquisition function to favor the good direction $+d$ would be an interesting idea for a risk-sensitive BO algorithm.

C) Finally, the monotonic behavior is very linked to the chosen learning rate. Making it harder to compare the behavior of the algorithms.


==> rebuttals/R4.tex <==
### Reviewer 4 ###

> (1) The paper is somewhat dense and difficult to parse.

We have updated Section 4 for simpler exposition. Please let us know if the paper is clearer and if there are any other parts of the paper that you would like to be clarified.

> (2) Empirical results are fine but could be stronger.

We would like to point out that our algorithm consistently outperforms the MPD baseline, which, to the best of our knowledge, is the state-of-the-art algorithm in Bayesian Optimization (BO) for Reinforcement Learning (RL). Notably, our mean function can improve all potential future BO methods when applied to continuous RL problems.

Also, we would like to point out that despite performing slightly worse than ARS in Hopper and Halfcheetah, the gap between our method and ARS is never large in ARS' favor. In contrast, on the higher dimensional tasks that are Walker2d and Ant, our method largely outperforms ARS.

> (3) I am a little bit worried about the assumption of a linear policy; it was unclear to me if this was for exposition, or a constraint on the algorithm. Could you clarify? 

Our theoretical analysis and methodology is not dependent on the linear policy assumption. Assumption 3.2 requires the policy to be Lipschitz and this includes richer class of policies including the linear ones (e.g. a ReLU neural network can be Lipschitz).

We choose to benchmark our algorithm using linear policies for two reasons:

1) RL with deterministic linear policies is a standard benchmark for the Bayesian optimization setting [1,2,3]. 

2) For computational considerations, BO cannot scale to the thousands of dimensions required for a neural network actor. At least, not with the standard algorithms.

> 4. I see that you assume that you have access to J, d, and Q, but not more granular information about observed s,a,r,s' sequences. Why is that? Is that just an assumption that could be relaxed, and if so, would the more granular information be useful in constructing better GP posteriors?

We train the Q-function in the classical way on the available transition data (s,a,r,s') collected from the rolled-out trajectories. Thank you for pointing out the lack of clarity. We make this point clearer in the revision of Algorithm (1).

> (5) You combine the Q-experts using a softmax of $\exp(R^2)$ terms. This seems somewhat ad hoc. Is there a principled reason for this choice?

Our aggregation scheme for critics is an adoption of the Follow The Regularized Leader (FTRL) algorithm to average our critics using softmax weighting and $R^2$ as the goodness-of-fit function [4]. We clarify this point in the revised draft. We would also like to point out that the ablation study benchmarks a variant of our algorithm with uniform weighting of the Q-experts (label Ensemble+R in Figure 4).

> (6) Resetting the least-performing critic also seems like an ad-hoc choice. Is there a principled reason for it?
 
In practice, we noticed some high variance between different runs when using a single critic. This was due to the critic neural network losing plasticity as discussed in the primacy bias paper. Resetting critics also helps decorrelating their predictions, which is useful for ensemble-based methods. In the ablation study, we compare our algorithm to an ablated version that removes the resetting of critics (label Softmax in Figure 4). We hope this makes a sufficiently convincing argument about the practical use of this choice.

[1] Müller, Sarah, Alexander von Rohr, and Sebastian Trimpe. "Local policy search with Bayesian optimization." Advances in Neural Information Processing Systems 34 (2021): 20708-20720.

[2] Nguyen, Quan, et al. "Local Bayesian optimization via maximizing probability of descent." Advances in neural information processing systems 35 (2022): 13190-13202.

[3] Eriksson, David, et al. "Scalable global optimization via local Bayesian optimization." Advances in neural information processing systems 32 (2019).

[4] Cesa-Bianchi, Nicolo, and Gábor Lugosi. Prediction, learning, and games. Cambridge university press, 2006.

==> rebuttals/R5.tex <==
### Reviewer 5 ###

> (1) Quite a lot of prior knowledge is required to understand this paper. I am not immediately familarly with BO methods for RL, perhaps some more intuition for comparison to more familiar RL methods may be helpful for the average RL practitioner.

We agree with the reviewer, we chose the MPD algorithm which adds another layer on top of the usual BO algorithms for two reasons. First, it is the state-of-the-art method in BO. The second is that MPD is a First Order BO method which allows us to derive Corollary (3.3.1) which bridges the gap between BO and RL methods.

Our work builds on MPD, which is a local Bayesian optimization method. This line of research is very recent, and combines Bayesian optimization with gradient descent. Our work specializes these methods to RL (prior work was completely black-box and could be applied to any domain) by using a learned Q-function in the Gaussian process prior. At an intuitive level, our method can be seen as a policy gradient method [1], where Bayesian optimization techniques are used to select in a clever way which the batch deterministic policies that we will rollout to collect transitions from the environment and hence explore.  

> (2) I am not familiar with Lipschitz MDPs, presumable the reward function is Lipschitz bounded, but what of the transition functions and policies? Is there a natural way of bounding these that makes sense?

For a Lipschitz MDP, the transition dynamics is Lipschitz continuous w.r.t. Wasserstein distance. The same applies to the policies whose actions are smooth w.r.t to the state. This assumption has been used in literature [2] to bound the residual term for deterministic policies. We refer the reviewer to Assumptions 3.1 and 3.2 for further details.
Though our theoretical results rely on this assumption, we do not need to compute the Lipschitz constants for our algorithm, as demonstrated by our experimental results for MuJoCo.

> (3) What are the key differences between your approach and the baselines considered in this paper?

Our main baseline is the MPD algorithm. Our algorithm ABS can be seen as a variant where we improve the mean function of the Gaussian Process, usually taken to be a constant, to the advantage mean function that we develop.

The second baseline ARS is a standard evolutionary strategy algorithm. We are different from ARS in that our algorithm will be sampling adaptively the "acquisition points" using the acquisition function, whereas ARS samples the acquisition points according to a fixed distribution. ARS also follows a different descent direction for the gradient.

> (4) What are the reasons for only considering deterministic policies?

Our analysis and methodology generalize to stochastic policies (except Equation (7)).

We choose to benchmark our algorithm using linear policies for 3 reasons:

1) In our study, we focus on learning good policies while using exclusively deterministic policies for exploration. This approach is particularly beneficial when interacting with physical systems, where the implementation of deterministic policies is often more desirable.

2) RL with deterministic linear policies is a standard benchmark for the Bayesian optimization setting [3,4,5]. 

3) Deterministic policies allow for less noise in the policy evaluation compared to a stochastic policy and hence fewer rollouts are necessary to estimate the return of a policy $\pi$. 

[1] Sutton, Richard S., and Andrew G. Barto. Reinforcement learning: An introduction. MIT press, 2018.

[2] Saleh, Ehsan, et al. "Truly Deterministic Policy Optimization." Advances in Neural Information Processing Systems 35 (2022): 8469-8482.

[3] Müller, Sarah, Alexander von Rohr, and Sebastian Trimpe. "Local policy search with Bayesian optimization." Advances in Neural Information Processing Systems 34 (2021): 20708-20720.

[4] Nguyen, Quan, et al. "Local Bayesian optimization via maximizing probability of descent." Advances in neural information processing systems 35 (2022): 13190-13202.

[5] Eriksson, David, et al. "Scalable global optimization via local Bayesian optimization." Advances in neural information processing systems 32 (2019).


==> rebuttals/general.tex <==
We thank all Reviewers for their valuable feedback. We have uploaded a revised draft in which we make some changes to address the concerns and misunderstandings that have been raised.

As a summary, we have:

- Added a paragraph on the role of Corollary 3.3.1 which gives a better intuition of the interplay between the GP and the Q-function approximator. 

- Improved Section 4 to make the proposed validation and test metrics clearer.

- Removed the smoothing used in the initial version of Figure 2, and added a histogram of the distribution of validation and test scores in the appendix to make the interpretation of our results easier.

- Added a summary of the results at the end of Section 5.2.

- Fixed the various typos and clarified several claims following the reviewers' feedback.

- We have updated the figures to improve readability (the results are unchanged).



==> sections/rebuttals.tex <==
### General answer 

Q1) performance us vs MPD we're always better.

us vs ARS normalization + when we beat them we beat them by a margin.

### Reviewer 1 ###

> There is no comparison with one of the frequently used model-free RL methods with bootstrapping.

> The term "deterministic exploration" requires an explanation.

> Why was a comparison with bootstrapping-based methods such as NFQ [4], DQN [5], SAC [6], etc. omitted?

We thank the reviewer for raising these questions. Which we believe are connected to the ambiguity of the term "deterministic exploration".  

The main point of our paper is to learn good policies using only deterministic policies . We take the reviewer's opinion into account and accentuate more the 
% We want to remark that the model free RL methods with bootstrapping hinge on a stochastic actor, including DPG and its variants.


> The presentation does not classify the approach clearly enough in the very broad field of RL algorithms.

"CITE PAPER AGAIN"









